Findings of the TSAR-2022 Shared Task on Multilingual Lexical Simplification

We report findings of the TSAR-2022 shared task on multilingual lexical simplification, organized as part of the Workshop on Text Simplification, Accessibility, and Readability TSAR-2022 held in conjunction with EMNLP 2022. The task called the Natural Language Processing research community to contribute with methods to advance the state of the art in multilingual lexical simplification for English, Portuguese, and Spanish. A total of 14 teams submitted the results of their lexical simplification systems for the provided test data. Results of the shared task indicate new benchmarks in Lexical Simplification with English lexical simplification quantitative results noticeably higher than those obtained for Spanish and (Brazilian) Portuguese.

==> TSAR_2022_Results_Discussion_TO_MAIN_TEXT.tex <==
% working on the results
In the following subsections we describe the results obtained by the participant teams for each of the tracks in the TSAR 2022 Multilingual Lexical Simplification shared task.\footnote{Please note that official results can also be queried at \url{https://taln.upf.edu/pages/tsar2022-st/#results}}  Note that we will base our description on the ranking obtained by sorting submissions according to the ACC@1 metric as well as summarizing methods for which a paper has been submitted and accepted for the Shared Task (see Section \ref{sec:systems}). 

We also provided an extended version of the results,\footnote{\url{https://github.com/LaSTUS-TALN-UPF/TSAR-2022-Shared-Task/tree/main/results/extended}} which included ACC@1, Potential@k, MAP@k, macro-averaged Precision@k, macro-averaged Recall@k, and Accuracy@k@top1, for k $\in$ \{1, 2, ..., 10\}.
Precision@k and Recall @k were defined as follows:
\begin{itemize}

\item {\bf Precision@k}: the percentage of $k$ top-ranked substitutes that are present also in the gold data; 
 \item {\bf Recall@k}: the percentage of substitutions provided in the gold data that are included in the top $k$ generated substitutions.
\end{itemize}
\\


Overall, we observe that several systems achieved new state-of-the-art results  in the different tracks overtaking a previous competitive Neural Language Model for lexical simplification (LSBert).

\subsection{English Track}
In table \ref{table:results_en} the results for English are presented sorted by ACC@1.\footnote{Note that the data to sort the results is available at \url{https://github.com/LaSTUS-TALN-UPF/TSAR-2022-Shared-Task/tree/main/results/official}} In this track, and of the 31 submitted runs, only four (from 3 teams: UniHD, MANTIS, and UoM\&MMU) performed better than the LSBert baseline according to ACC@1. Moreover, UniHD run number 2 achieved the best performance  in all the reported metrics. 
UniHD run number 2 outperforms the other teams' systems in more than 15 points in ACC@1 achieving a score of 0.8096 in this metric. This indicates that it is able to retrieve a correct synonym in the 80,96\% of instances of the dataset.
Moreover, UniHD's run number 2 achieves a 99,46\% of Potential@10. This indicates that it has the potential to retrieve at least one correct substitution in the top-10 predictions of almost all the instances.
In fact, it achieves 0.9624 in Potential@3 metric, which is almost nine points higher than the second best official result (MANTIS with 0.8900) and indicates also a great performance obtaining at least one correct substitution in the top-3 predictions.

It is important to highlight that the UniHD's system relies on a pre-trained {\em pay-per-query}  GPT-3 model to obtain candidate substitutions by prompting the  model with 6 versions of zero, one, and two shot prompts, based on the provided trial data,  finally combining the predicted candidate ranks to select the best substitutions. 
In contrast, team MANTIS relied on a freely available masked language model to obtain substitutions and an adaptation of the ranking procedure of LSBert.  While UoM\&MMU also relying on  freely available pre-trained masked language models fine tuned  with prompts to select the most appropriate substitutes and filtering substitution candidates by checking several resources (e.g. WordNet, corpora).  Also noticeable in the results of the task is that several ``neural'' systems under-perform the ``non-neural'' TUNER baseline in terms of ACC@1.  
Overall, it seems that the use of pre-trained masked language models fine-tuned to the task together with extra lexical resources or corpora produce very competitive approaches.

\subsection{Portuguese Track}
Table \ref{table:results_pt}, presents the results for Portuguese, also sorted by ACC@1.  In this track, and of the 14 submitted runs, only two (from two teams:  GMU-WLV and CENTAL) performed better than the LSBert baseline (as observed in the table, one team performed equally to LSBert in terms of ACC@1, but worst in the other metrics). The displayed results indicate that there is a clear top performing (considering all metrics)  system produced by team GMU-WLV. Surprisingly, they have relied on a simple approach to substitute generation and ranking by adopting a pre-trained Portuguese masked language model,  BERTimbau \cite{souza2020bertimbau}. The second best performing system according to ACC@1 is by the CENTAL team which also relied on a pre-trained masked language model in which several strategies were used to provide context to the target sentence, followed by a ranking procedure based on voting.  Similar as in the English track, in this track, several systems  under-perform, in terms of ACC@1,  the shared task non-neural TUNER baseline.

\subsection{Spanish Track}
Results for the Spanish track are presented in Table~\ref{table:results_es}. The systems' runs are sorted by ACC@1. Several systems outperformed the LSBert baseline. In particular, the PresiUniv team produced two competitive approaches which ranked first and third (tied with team UoM\&MMU). However, the approach did not reach top performance in several of the official metrics. The PresiUniv lexical simplifier relies on a masked language model approach for substitute selection combined with a word-embbeding similarity model for meaning  preservation and a filtering stage based on POS-tagging. The  UoM\&MMU, GMU-WLV and CENTAL (with approaches already described for English or Portuguese)  also performed well in the Spanish track, with UoM\&MMU and GMU-WLV achieving top scores for some of the metrics. The PolyU-CBS team produced a competitive system which  used a Spanish specific masked language model to generate substitutes and a ranking based on a combination of sentence language model probabilities and word-embedding similarities. Best performing systems in this track rely on Spanish-specific masked language models, corpus-based information, language model prompts, and  syntactic information, among others.

